MVHuman: Tailoring 2D Diffusion with Multi-view Sampling For Realistic 3D Human Generation

Recent months have witnessed rapid progress in 3D generation based on diffusion models. Most advances require fine-tuning existing 2D Stable Diffsuions into multi-view settings or tedious distilling operations and hence fall short of 3D human generation due to the lack of diverse 3D human datasets. We present an alternative scheme named MVHuman to generate human radiance fields from text guidance, with consistent multi-view images directly sampled from pre-trained Stable Diffsuions without any fine-tuning or distilling. Our core is a multi-view sampling strategy to tailor the denoising processes of the pre-trained network for generating consistent multi-view images. It encompasses view-consistent conditioning, replacing the original noises with ``consistency-guided noises'', optimizing latent codes, as well as utilizing cross-view attention layers. With the multi-view images through the sampling process, we adopt geometry refinement and 3D radiance field generation followed by a subsequent neural blending scheme for free-view rendering. Extensive experiments demonstrate the efficacy of our method, as well as its superiority to state-of-the-art 3D human generation methods.

==> sec/Overview.tex <==


%
\section{Overview}
\papername enables generating 3D realistic human by exploiting as much as possible the original generation ability of the pre-trained stable diffusion model and ControlNet without any fine-tuning or extra networks. 
%
We first obtain human mesh along with human priors, then multi-view consistent images are denoised jointly from views on designed tracks. Finally, optimized mesh and free-view render results are reconstructed from images. 
%
We briefly discuss each step below, and provide detailed explanation in Sec.~\ref{sec:algorithm}

\noindent{\bf Geometry and Human Prior.}
As illustrated in Fig.~\ref{fig:fig_overview},
%
\papername obtain human meshes and priors in two ways.
%
One way is to generate a human mesh from a prompt. We combine the SD model and a single-view reconstruction method ECON~\cite{xiu2023econ} which already provides a SMPL-X along with mesh.
%
The other way is to fit a SMPL-X to a scanned human mesh directly.
%
From both ways, we get a mesh and a fitted SMPL-X as human prior.

\noindent{\bf Multi-view Sampling Process.}
As shown in Fig.~\ref{fig:fig_overview}, we set up a scene having views on two circular tracks. From each view, we obtain consistent controlling conditions from preprocessing. 
%
We then modify a multi-view sampling process to generate multi-view consistent images with the SD model.
% 
%
First, for the sampling of latent code at each view, we propose a novel consistency-guided noise in order to have consistency in image space.
%
Then, we optimize the latent codes of all views for explicit constraints.
%
We further manipulate the input features to the self-attention block by injecting the feature from the facing view to all other views.
% 

\noindent{\bf Geometry Optimization and Free-view Render.}
To make geometry details as rich as texture details of generated images, we further predict normal images from RGB images and apply a geometry optimization on original mesh. 
%
To obtain free-view rendering, we combine NeRF with Image-based rendering to get high-quality results.


\begin{figure*}[t] 
    \vspace{-1ex}
	\begin{center} 
		\includegraphics[width=\linewidth]{imgs/overview_v2.pdf} 
	\end{center} 
% 	\vspace{-2ex}
    \vspace{-20pt}
    \caption{The Overview of our MVHuman pipeline. Our approach consists of three steps. The first step includes two alternative modules to obtain a mesh and a fitted SMPL-X as human prior (Sec.~\ref{sec:geometry_init}). The second step perform a joint denoising process to generate view consistent images (Sec.~\ref{sec:multiview_sampling}). The third step includes three module to enable high-quality free-view rendering.} 
	\label{fig:fig_overview} 
	\vspace{-10pt}
\end{figure*} 

